Waveform Design for Mutual Interference Mitigation in Automotive Radar

The mutual interference between similar radar systems can result in reduced radar sensitivity and increased false alarm rates. To address the synchronous and asynchronous interference mitigation problems in similar radar systems, we first propose herein two slow-time coding schemes to modulate the pulses within a coherent processing interval (CPI) for a single-input-single-output (SISO) scenario. Specifically, the first coding scheme relies on Doppler shifting and the second one is devised based on an optimization approach. We further extend our discussion to the more general case of multiple-input-multiple-output (MIMO) radars and propose an efficient algorithm to design waveforms to mitigate mutual interference in such systems. The proposed coding schemes are computationally efficient in practice and the incorporation of the coding schemes requires only a slight modification of the existing systems. Our numerical examples indicate that the proposed coding schemes can reduce the interference power level in a desired area of the cross-ambiguity function significantly.

==> MIMO Interference Mitigation for Automotive Radar/symbols.tex <==
%% Short symbol commands for LaTex
\usepackage{amsmath}
\usepackage{algpseudocode}
\usepackage{amsthm}
\usepackage{dsfont}
\usepackage{algorithm}
\usepackage{thmtools}
\usepackage{amssymb}
\usepackage[dvipsnames]{xcolor}
\usepackage{todonotes}



\def \Author{Arindam~Bose}
\def \Version{2.0.16}
\def \Update{\today}

% Lower case bold English alphabets
\def\ba{\boldsymbol{a}}
\def\bb{\boldsymbol{b}}
\def\bc{\boldsymbol{c}}
\def\bd{\boldsymbol{d}}
\def\be{\boldsymbol{e}}
\def\bdf{\boldsymbol{f}}
\def\bg{\boldsymbol{g}}
\def\bh{\boldsymbol{h}}
\def\bi{\boldsymbol{i}}
\def\bj{\boldsymbol{j}}
\def\bk{\boldsymbol{k}}
\def\bl{\boldsymbol{l}}
\def\bm{\boldsymbol{m}}
\def\bn{\boldsymbol{n}}
\def\bo{\boldsymbol{o}}
\def\bp{\boldsymbol{p}}
\def\bq{\boldsymbol{q}}
\def\br{\boldsymbol{r}}
\def\bs{\boldsymbol{s}}
\def\bt{\boldsymbol{t}}
\def\bu{\boldsymbol{u}}
\def\bv{\boldsymbol{v}}
\def\bw{\boldsymbol{w}}
\def\bx{\boldsymbol{x}}
\def\by{\boldsymbol{y}}
\def\bz{\boldsymbol{z}}

% Upper case bold English alphabets
\def\bA{\boldsymbol{A}}
\def\bB{\boldsymbol{B}}
\def\bC{\boldsymbol{C}}
\def\bD{\boldsymbol{D}}
\def\bE{\boldsymbol{E}}
\def\bF{\boldsymbol{F}}
\def\bG{\boldsymbol{G}}
\def\bH{\boldsymbol{H}}
\def\bI{\boldsymbol{I}}
\def\bJ{\boldsymbol{J}}
\def\bK{\boldsymbol{K}}
\def\bL{\boldsymbol{L}}
\def\bN{\boldsymbol{N}}
\def\bM{\boldsymbol{M}}
\def\bO{\boldsymbol{O}}
\def\bP{\boldsymbol{P}}
\def\bQ{\boldsymbol{Q}}
\def\bR{\boldsymbol{R}}
\def\bS{\boldsymbol{S}}
\def\bT{\boldsymbol{T}}
\def\bU{\boldsymbol{U}}
\def\bV{\boldsymbol{V}}
\def\bW{\boldsymbol{W}}
\def\bX{\boldsymbol{X}}
\def\bY{\boldsymbol{Y}}
\def\bZ{\boldsymbol{Z}}

% Bold Greek alphabets
\def\balpha{\boldsymbol{\alpha}}
\def\bbeta{\boldsymbol{\beta}}
\def\bgamma{\boldsymbol{\gamma}}
\def\bGamma{\boldsymbol{\Gamma}}
\def\bdelta{\boldsymbol{\delta}}
\def\bDelta{\boldsymbol{\Delta}}
\def\bepsilon{\boldsymbol{\epsilon}}
\def\bvarepsilon{\boldsymbol{\varepsilon}}
\def\bzeta{\boldsymbol{\zeta}}
\def\bdeta{\boldsymbol{\eta}}
\def\btheta{\boldsymbol{\theta}}
\def\bvartheta{\boldsymbol{\vartheta}}
\def\bTheta{\boldsymbol{\Theta}}
\def\biota{\boldsymbol{\iota}}
\def\bkappa{\boldsymbol{\kappa}}
\def\blambda{\boldsymbol{\lambda}}
\def\bLambda{\boldsymbol{\Lambda}}
\def\bmu{\boldsymbol{\mu}}
\def\bnu{\boldsymbol{\nu}}
\def\bxi{\boldsymbol{\xi}}
\def\bXi{\boldsymbol{\Xi}}
\def\bpi{\boldsymbol{\pi}}
\def\bPi{\boldsymbol{\Pi}}
\def\brho{\boldsymbol{\rho}}
\def\bvarrho{\boldsymbol{\varrho}}
\def\bsigma{\boldsymbol{\sigma}}
\def\bSigma{\boldsymbol{\Sigma}}
\def\btau{\boldsymbol{\tau}}
\def\bupsilon{\boldsymbol{\upsilon}}
\def\bUpsilon{\boldsymbol{\Upsilon}}
\def\bphi{\boldsymbol{\phi}}
\def\bvarphi{\boldsymbol{\varphi}}
\def\bPhi{\boldsymbol{\Phi}}
\def\bchi{\boldsymbol{\chi}}
\def\bpsi{\boldsymbol{\psi}}
\def\bPsi{\boldsymbol{\Psi}}
\def\bomega{\boldsymbol{\omega}}
\def\bOmega{\boldsymbol{\Omega}}

% Mathbf lower case English alphabets
\def\mba{\mathbf{a}}
\def\mbb{\mathbf{b}}
\def\mbc{\mathbf{c}}
\def\mbd{\mathbf{d}}
\def\mbe{\mathbf{e}}
\def\mbf{\mathbf{f}}
\def\mbg{\mathbf{g}}
\def\mbh{\mathbf{h}}
\def\mbi{\mathbf{i}}
\def\mbj{\mathbf{j}}
\def\mbk{\mathbf{k}}
\def\mbl{\mathbf{l}}
\def\mbm{\mathbf{m}}
\def\mbn{\mathbf{n}}
\def\mbo{\mathbf{o}}
\def\mbp{\mathbf{p}}
\def\mbq{\mathbf{q}}
\def\mbr{\mathbf{r}}
\def\mbs{\mathbf{s}}
\def\mbt{\mathbf{t}}
\def\mbu{\mathbf{u}}
\def\mbv{\mathbf{v}}
\def\mbw{\mathbf{w}}
\def\mbx{\mathbf{x}}
\def\mby{\mathbf{y}}
\def\mbz{\mathbf{z}}

% Mathbf upper case English alphabets
\def\mbA{\mathbf{A}}
\def\mbB{\mathbf{B}}
\def\mbC{\mathbf{C}}
\def\mbD{\mathbf{D}}
\def\mbE{\mathbf{E}}
\def\mbF{\mathbf{F}}
\def\mbG{\mathbf{G}}
\def\mbH{\mathbf{H}}
\def\mbI{\mathbf{I}}
\def\mbJ{\mathbf{J}}
\def\mbK{\mathbf{K}}
\def\mbL{\mathbf{L}}
\def\mbM{\mathbf{M}}
\def\mbN{\mathbf{N}}
\def\mbO{\mathbf{O}}
\def\mbP{\mathbf{P}}
\def\mbQ{\mathbf{Q}}
\def\mbR{\mathbf{R}}
\def\mbS{\mathbf{S}}
\def\mbT{\mathbf{T}}
\def\mbU{\mathbf{U}}
\def\mbV{\mathbf{V}}
\def\mbW{\mathbf{W}}
\def\mbX{\mathbf{X}}
\def\mbY{\mathbf{Y}}
\def\mbZ{\mathbf{Z}}

% Caligraphy upper case English alphabets
\def\calA{\mathcal{A}}
\def\calB{\mathcal{B}}
\def\calC{\mathcal{C}}
\def\calD{\mathcal{D}}
\def\calE{\mathcal{E}}
\def\calF{\mathcal{F}}
\def\calG{\mathcal{G}}
\def\calH{\mathcal{H}}
\def\calI{\mathcal{I}}
\def\calJ{\mathcal{J}}
\def\calK{\mathcal{K}}
\def\calL{\mathcal{L}}
\def\calM{\mathcal{M}}
\def\calN{\mathcal{N}}
\def\calO{\mathcal{O}}
\def\calP{\mathcal{P}}
\def\calQ{\mathcal{Q}}
\def\calR{\mathcal{R}}
\def\calS{\mathcal{S}}
\def\calT{\mathcal{T}}
\def\calU{\mathcal{U}}
\def\calV{\mathcal{V}}
\def\calW{\mathcal{W}}
\def\calX{\mathcal{X}}
\def\calY{\mathcal{Y}}
\def\calZ{\mathcal{Z}}

% Numbers
\def\bzero{\boldsymbol{0}}
\def\bone{\boldsymbol{1}}

% Sets and notations
\newcommand{\binaryB}[1][]{\mathds{B}^{#1}}
\newcommand{\complexC}[1][]{\mathds{C}^{#1}}
\newcommand{\expecE}[1]{\mathds{E}\left\{{#1}\right\}}
\newcommand{\naturalN}[1][]{\mathds{N}^{#1}}
\newcommand{\probP}[1]{\mathds{P}\mathrm{r}\left\{{#1}\right\}}
\newcommand{\rationalQ}[1][]{\mathds{Q}^{#1}}
\newcommand{\realR}[1][]{\mathds{R}^{#1}}
\newcommand{\realRp}[1][]{\mathds{R}_{+}^{#1}}
\newcommand{\realRn}[1][]{\mathds{R}_{-}^{#1}}
\newcommand{\integerZ}[1][]{\mathds{Z}^{#1}}

% Matrix terms
\def\tr#1{\mathrm{tr}\left(#1\right)}
\def\Tr#1{\mathrm{Tr}\left(#1\right)}
\def\vec#1{\mathrm{vec}\left(#1\right)}
\def\diag#1{\mathrm{diag}\left(#1\right)}
\def\Diag#1{\mathrm{Diag}\left(#1\right)}
\def\bdiag#1{\mathbf{diag}\left(#1\right)}
\def\cov#1{\mathrm{cov}\left(#1\right)}
\def\Cov#1{\mathrm{Cov}\left(#1\right)}
\def\bcov#1{\mathbf{cov}\left(#1\right)}

% Misc
\def\asin#1{\sin^{-1}\left(#1\right)}
\def\acos#1{\cos^{-1}\left(#1\right)}
\def\atan#1{\tan^{-1}\left(#1\right)}
\def\acsc#1{\csc^{-1}\left(#1\right)}
\def\asec#1{\sec^{-1}\left(#1\right)}
\def\acot#1{\cot^{-1}\left(#1\right)}
\newcommand{\parderiv}[3][]{\dfrac{\partial^{#1} #2}{\partial #3^{#1}}}
\newcommand{\deriv}[3][]{\dfrac{d^{#1} #2}{d#3^{#1}}}
\def\implies{\Rightarrow}
\def\half{\frac{1}{2}}
\def\roothalf{\frac{1}{\sqrt{2}}}
\def\third{\frac{1}{3}}
\def\quarter{\frac{1}{4}}
\def\fourth{\frac{1}{4}}
\def\fifth{\frac{1}{5}}
\def\threequarter{\frac{3}{4}}
\newcommand{\ejomg}[1][]{e^{j#1\omega}}
\newcommand{\ejnomg}[1][]{e^{-j#1\omega}}
\newcommand{\zinv}[1][]{z^{\ifx&#1&-1\else-#1\fi}}
\def\sgn#1{\mathrm{sgn}\left(#1\right)}
\def\sign#1{\mathrm{sign}\left(#1\right)}
\def\csign#1{\mathrm{csign}\left(#1\right)}
\def\deg{^\circ}
\def\Oh#1{\mathcal{O}\left(#1\right)}
\def\oh#1{o\left(#1\right)}
\def\d#1{\mathrm{d}#1}
\def\st{~\mathrm{s.t.}~}
\def\ow{~\mathrm{otherwise}}
\def\ew{~\mathrm{elsewhere}}
\def\eg{\textit{e.g.}}
\def\ie{\textit{i.e.}}
\def\wrt{\textit{w.r.t.~}}
\def\etal{\textit{et al.~}}
\def\etc{\textit{etc.~}}
\def\viz{\textit{viz.}}
\def\conv{\circledast}
\def\ord#1{^\text{#1}}
\def\eig#1{\mathrm{eig}\left(#1\right)}

% Basic text colors
\def\white#1{\textcolor{white}{#1}}
\def\black#1{\textcolor{black}{#1}}
\def\red#1{\textcolor{red}{#1}}
\def\green#1{\textcolor{green}{#1}}
\def\blue#1{\textcolor{blue}{#1}}
\def\cyan#1{\textcolor{cyan}{#1}}
\def\magenta#1{\textcolor{magenta}{#1}}
\def\yellow#1{\textcolor{yellow}{#1}}

% Special colors that comes with [dvipsnames] option in xcolor package
\def\Apricot#1{\textcolor{Apricot}{#1}}
\def\Aquamarine#1{\textcolor{Aquamarine}{#1}}
\def\Bittersweet#1{\textcolor{Bittersweet}{#1}}
\def\Black#1{\textcolor{Black}{#1}}
\def\Blue#1{\textcolor{Blue}{#1}}
\def\BlueGreen#1{\textcolor{BlueGreen}{#1}}
\def\BlueViolet#1{\textcolor{BlueViolet}{#1}}
\def\BrickRed#1{\textcolor{BrickRed}{#1}}
\def\Brown#1{\textcolor{Brown}{#1}}
\def\BurntOrange#1{\textcolor{BurntOrange}{#1}}
\def\CadetBlue#1{\textcolor{CadetBlue}{#1}}
\def\CarnationPink#1{\textcolor{CarnationPink}{#1}}
\def\Cerulean#1{\textcolor{Cerulean}{#1}}
\def\CornflowerBlue#1{\textcolor{CornflowerBlue}{#1}}
\def\Cyan#1{\textcolor{Cyan}{#1}}
\def\Dandelion#1{\textcolor{Dandelion}{#1}}
\def\DarkOrchid#1{\textcolor{DarkOrchid}{#1}}
\def\Emerald#1{\textcolor{Emerald}{#1}}
\def\ForestGreen#1{\textcolor{ForestGreen}{#1}}
\def\Fuchsia#1{\textcolor{Fuchsia}{#1}}
\def\Goldenrod#1{\textcolor{Goldenrod}{#1}}
\def\Gray#1{\textcolor{Gray}{#1}}
\def\Green#1{\textcolor{Green}{#1}}
\def\GreenYellow#1{\textcolor{GreenYellow}{#1}}
\def\JungleGreen#1{\textcolor{JungleGreen}{#1}}
\def\Lavender#1{\textcolor{Lavender}{#1}}
\def\LimeGreen#1{\textcolor{LimeGreen}{#1}}
\def\Magenta#1{\textcolor{Magenta}{#1}}
\def\Mahogany#1{\textcolor{Mahogany}{#1}}
\def\Maroon#1{\textcolor{Maroon}{#1}}
\def\Melon#1{\textcolor{Melon}{#1}}
\def\MidnightBlue#1{\textcolor{MidnightBlue}{#1}}
\def\Mulberry#1{\textcolor{Mulberry}{#1}}
\def\NavyBlue#1{\textcolor{NavyBlue}{#1}}
\def\OliveGreen#1{\textcolor{OliveGreen}{#1}}
\def\Orange#1{\textcolor{Orange}{#1}}
\def\OrangeRed#1{\textcolor{OrangeRed}{#1}}
\def\Orchid#1{\textcolor{Orchid}{#1}}
\def\Peach#1{\textcolor{Peach}{#1}}
\def\Periwinkle#1{\textcolor{Periwinkle}{#1}}
\def\PineGreen#1{\textcolor{PineGreen}{#1}}
\def\Plum#1{\textcolor{Plum}{#1}}
\def\ProcessBlue#1{\textcolor{ProcessBlue}{#1}}
\def\Purple#1{\textcolor{Purple}{#1}}
\def\RawSienna#1{\textcolor{RawSienna}{#1}}
\def\Red#1{\textcolor{Red}{#1}}
\def\RedOrange#1{\textcolor{RedOrange}{#1}}
\def\RedViolet#1{\textcolor{RedViolet}{#1}}
\def\Rhodamine#1{\textcolor{Rhodamine}{#1}}
\def\RoyalBlue#1{\textcolor{RoyalBlue}{#1}}
\def\RoyalPurple#1{\textcolor{RoyalPurple}{#1}}
\def\RubineRed#1{\textcolor{RubineRed}{#1}}
\def\Salmon#1{\textcolor{Salmon}{#1}}
\def\SeaGreen#1{\textcolor{SeaGreen}{#1}}
\def\Sepia#1{\textcolor{Sepia}{#1}}
\def\YellowOrange#1{\textcolor{YellowOrange}{#1}}
\def\SkyBlue#1{\textcolor{SkyBlue}{#1}}
\def\SpringGreen#1{\textcolor{SpringGreen}{#1}}
\def\Tan#1{\textcolor{Tan}{#1}}
\def\TealBlue#1{\textcolor{TealBlue}{#1}}
\def\Thistle#1{\textcolor{Thistle}{#1}}
\def\Turquoise#1{\textcolor{Turquoise}{#1}}
\def\Violet#1{\textcolor{Violet}{#1}}
\def\VioletRed#1{\textcolor{VioletRed}{#1}}
\def\White#1{\textcolor{White}{#1}}
\def\WildStrawberry#1{\textcolor{WildStrawberry}{#1}}
\def\Yellow#1{\textcolor{Yellow}{#1}}
\def\YellowGreen#1{\textcolor{YellowGreen}{#1}}
\def\YellowOrange#1{\textcolor{YellowOrange}{#1}}

% Theorem-like environments (defs, lemmas numbered like Theorems)
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{example}{Example}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\declaretheorem[style=definition,name=Remark,qed=$\blacksquare$]{remark}

\usepackage{xpatch}
\makeatletter
\xpatchcmd{\@thm}{\thm@headpunct{.}}{\thm@headpunct{}}{}{}
\makeatother

% algorithms
%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Initialize:}}
\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}
\algnewcommand\algorithmicoutput{\textbf{Output:}}
\algnewcommand\Output{\item[\algorithmicoutput]}
\algnewcommand\algorithmicinit{\textbf{Initialize:}}
\algnewcommand\Init{\item[\algorithmicinit]}
\def\Print#1{\textbf{print}~#1}
\def\To{\textbf{to}~}

% underbrace inside a matrix environment
\newcommand\undermat[2]{
	\makebox[0pt][l]{${\underbrace{\hphantom{
					\begin{matrix}#1\end{matrix}}}_{\text{$#2$}}}$}#1}
				
% todo stuff
\def\TODO#1{\todo[inline, color=red!40]{#1}}
\def\DONE#1{\todo[inline, color=green!40]{#1}}
